Relational Memory: Native In-Memory Accesses on Rows and Columns

Analytical database systems are typically designed to use a column-first data layout to access only the desired fields. On the other hand, storing data row-first works great for accessing, inserting, or updating entire rows. Transforming rows to columns at runtime is expensive, hence, many analytical systems ingest data in row-first form and transform it in the background to columns to facilitate future analytical queries. How will this design change if we can always efficiently access only the desired set of columns? To address this question, we present a radically new approach to data transformation from rows to columns. We build upon recent advancements in embedded platforms with re-programmable logic to design native in-memory access on rows and columns. Our approach, termed Relational Memory, relies on an FPGA- based accelerator that sits between the CPU and main memory and transparently transforms base data to any group of columns with minimal overhead at runtime. This design allows accessing any group of columns as if it already exists in memory. We implement and deploy Relational Memory in real hardware, and we show that we can access the desired columns up to 1.63x faster than accessing them from their row-wise counterpart, while matching the performance of a pure columnar access for low projectivity, and outperforming it by up to 1.87x as projectivity (and tuple re-construction cost) increases. Moreover, our approach can be easily extended to support offloading of a number of operations to hardware, e.g., selection, group by, aggregation, and joins, having the potential to vastly simplify the software logic and accelerate the query execution.

==> docs/4-design.tex <==
\newcommand{\profc}{\texttt{profctl}\xspace}
\newcommand{\profv}{\texttt{profvm}\xspace}
\newcommand{\staller}{Staller}
\newcommand{\requestor}{Requestor}
\newcommand{\fetch}{Fetch Unit}
\newcommand{\bypass}{Monitor Bypass}
\newcommand{\extcol}{Column Extractor}
\newcommand{\reader}{AXI Reader}
\newcommand{\writer}{AXI Writer}


\section{Design}
\begin{figure*}[]
	\centering
	\includegraphics[width=0.95\textwidth]{figs/design}
	\caption{Block Diagram}
	\label{fig:design}
\end{figure*}

\todo{Here we will have one section that described Relational Memory and its design in detail.}

Building on the ability to implement and test PLIM modules today in commercial platforms, we focus on one of the data-intensive applications that can benefit the most from near-memory processing, namely database systems. Specifically, while traditionally analytical and transactional systems where two completely separate codebases with completely different designs, the increased blending of application requirements for hybrid transactional/analytical processing (HTAP) has created the need to bridge their differences. The most common one being the physical data layout between column-stores, row-stores or hybrid stores with groups of columns. To date, prior approaches propose different solutions from the software side. Here we propose a software-hardware co-design approach that allows efficient physical access row-wise, column-wise, or any intermediate hybrid using PLIM. This has transformative impact on data systems architectures.

A natural design choice in this sense is to place near-memory processing unit as close as possible to the actual memory storage. In traditional DRAM-based systems, this can translate to having a processor in each DRAM bank. On the other hand, for a workload that requires a more global view over memory, embedding a programmable processor in the DRAM controller may be more beneficial. At the same time, a co-processor capable of simultaneously controlling multiple DRAM channels is to be preferred to exploit further parallelism. Additionally, when tight coupling between I/O data streams and memory content is present, a programmable entity placed on the main interconnect could provide an important level of control to refine the organization of I/O data before it is stored in DRAM. It follows that a generic-enough architecture capable of minimizing the cost of data movement should include near-memory processors at multiple levels. These should not work independently, but rather cooperate such that only operations that cannot be efficiently performed at a lower level (closer to DRAM) are enacted in a higher-up level of the hierarchy (closer to CPUs).

\subsection{Design Challenges}
\subsection{\staller{}}
The core directly sends the read requests to the \staller{} in the form of read request address. Upon receiving this request, the \staller{} tries to trigger the \requestor{}. One key issue is that the core can issue multiple asynchronous requests to the \staller{}. The \staller{} handles these requests in the following way: when a request comes, the \staller{} checks if a cache line is ready. If it is not, the request is stalled for the time being (hence the name \textit{\staller{}}). The request will be served as soon as a cache line becomes ready.

\subsection{\requestor}
The main job of the \requestor{} is to calculate the inputs for the \fetch{} along with the corresponding SPM addresses. Based on the original read request address and other inputs (e.g. DB row width, DB row count, DB column size, and offset), the \requestor{} calculates 
the DRAM address, SPM address and data offsets for each \fetch{}. Offset and all addresses are considered in bytes. The details of these inputs are presented in Table~\ref{tab:input_requestor}.

%DB row width indicates the row size of the DB, DB row count is the number of rows to fetch from DB, offset is the position of the interested column within a row, and the DLEN indicates the size of the desired column. 

\begin{table}[]
\caption{Inputs of the \requestor}
\label{tab:input_requestor}
\resizebox{0.45\textwidth}{!}{%
\begin{tabular}{|l|c|l|}
\hline
\multicolumn{1}{|c|}{\textbf{Input}} & \multicolumn{1}{c|}{\textbf{Size (bytes)}} & \multicolumn{1}{c|}{\textbf{Description}}                                                 \\ \hline
BUS WIDTH                            & $16$                                         & Size of the BUS                                                                           \\ \hline
DB ROW WIDTH                         & $1 - 2^{16}$                                      & Row size of the DB                                                                        \\ \hline
DB ROW COUNT                         & $1 - 2^{16}$                                      & Number of rows in the DB                                                                  \\ \hline
Offset                               & $0-15$                                       & \begin{tabular}[c]{@{}l@{}}Position of the interested \\ column within a row\end{tabular} \\ \hline
DLEN                                 & $1-32$                                       & Size of the desired column                                                                \\ \hline
\end{tabular}%
}
\end{table}

In order to reduce the number of AXI transactions, the \requestor{} supports burst read and write when the data resides in multiple bus lines. The \requestor{} serially generates the addresses for the \fetch{}s
for all the DB rows. The \requestor{} can support upto 16 \fetch{}s. If all 
the \fetch{}s are busy, then the \requestor{} stops and waits for the transaction to be finished. The requestor keeps track of which \fetch{} is available via monitoring the ready signals from the \fetch{}s.

\subsection{\fetch}
\textcolor{blue}{work in progress}

Each \fetch{} is responsible for retrieving one fixed size chunk of data from the DRAM and then directing it to the designated place in SPM.

\Paragraph{\extcol{}}
\extcol{} resides in the \fetch{}. It receives the row data from DRAM and extracts the desired 
column from the row based on the inputs passed by the \requestor{}. If the target column spans across the multiple bus lines, it waits until all the column data is accumulated and indicates the validity of the output by setting the enable signal. Finally, the output column data is passed on to the \writer{}.

\Paragraph{\writer{}}
It generates an AXI transaction with an ID based on two information: (i) where the write will be performed inside the cache line, (ii) data offset. The id corresponds to the write address. As a result, upon receiving the acknowledgement, we can update the corresponding ``Table'' entry of the \bypass{}. 

AXI Writers embeds the write address in the write transaction ID; this is done so that the cache line\#(s) can be derived from the ID. \bypass{} updates the per cache-line counter upon receiving a Write Ack (on AXI channel B) with the number of valid bytes written to SPM. Ready bit sets (Fill Counter == 64 Bytes ).

Problem: Table could get really large. 

Solution: Track ready pages (4KB) in the SPM instead of ready cache-lines (64B).
 
\subsection{\bypass}
\bypass{}  keeps track of the SPM and makes sure writes are performed in the appropriate location inside the SPM. Whenever a cache line becomes ready, it signals the \staller{} about the corresponding cache line which is ready to be fetched. It does so by maintaining a ``Table'' where each entry corresponds to a cache line. Upon receiving a transaction, the \bypass{} updates the the number of bytes written to that cache line. Once it reaches some threshold, (e.g. whole cache line size), the \bypass{} enables the ``ready'' bit signaling the \staller{} that it can \textit{unstall}/\textit{unfreeze} the original request.
\subsection{Putting it All Together}
The core requests read requests with addresses to the \staller{}. Based on the availability of a cache line, that request is either served or stalled. The \requestor{} performs necessary calculations in order to calculate the DRAM address, SPM address and other inputs for the \fetch{}. It also keeps track of which \fetch{} is currently busy. The \fetch{} sends a ``fixed'' number of Burst DRAM transactions towards the DRAM. For each completed DRAM requests, data will be filtered in ``fixed'' number of FPGA cycles. This filtering is performed insider the \extcol{} module of the \fetch{}. The filtered data is then transferred to the SPM Write Master and will be written at the appropriate location. The AXI write responses are routed through the \bypass{} which signals the \staller{} to unfreeze the corresponding stalled transaction once a cache line is ready. A \textit{ready} signal will indicate if valid data of a size of cache line is available in the SPM.

==> docs/motivation.tex <==
\section{Motivating Example}\label{sec:motivation}


==> docs/notation.tex <==
%%%%% NOTATION COMMANDS %%%%

\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

\newcommand{\optarg}[1][]{%
  \ifthenelse{\isempty{#1}}%
             {}% if #1 is empty
             {_{#1}}% if #1 is not empty
}

\newcommand{\optpar}[1][]{%
  \ifthenelse{\isempty{#1}}%
             {}% if #1 is empty
             {(#1)}% if #1 is not empty
}

\newcommand{\sma}[1]{\ensuremath{#1}\xspace}

\newcommand{\cpunum}{\sma{m}}
\newcommand{\cpuind}{\sma{k}}
\newcommand{\cpu}[1][\cpuind]{\sma{CPU\optarg[#1]}}

\newcommand{\accnum}{\sma{a}}
\newcommand{\accind}{\sma{l}}
\newcommand{\acc}[1][\accind]{\sma{ACC\optarg[#1]}}

%% Maximum BW supported by the DDR
\newcommand{\bwcapr}[1][]{\sma{\widehat{b^r\optarg[#1]}}}
\newcommand{\bwcapw}[1][]{\sma{\widehat{b^w\optarg[#1]}}}
\newcommand{\bwcap}[1][]{\sma{\widehat{b\optarg[#1]}}}

%% BW Max for Reads and Writes
\newcommand{\maxbwr}{\sma{B^r}}
\newcommand{\bwmaxr}{\sma{\maxbwr}}

\newcommand{\maxbww}{\sma{B^w}}
\newcommand{\bwmaxw}{\sma{\maxbww}}

%% Max utilization
\newcommand{\util}{\sma{U}}
\newcommand{\maxutil}{\sma{\widehat{U}}}

%% Task notation
\newcommand{\tasknum}{\sma{n}}
\newcommand{\taskind}{\sma{i}}
\newcommand{\task}[1][\taskind]{\sma{\tau\optarg[#1]}}

\newcommand{\supenvind}{\sma{j}}

%% Envelope notation
\newcommand{\envset}[1][\taskind]{\sma{\mathcal{M}\optarg[#1]}}
\newcommand{\envel}[1][\supenvind]{\sma{M\optarg[#1]}}
\newcommand{\envlen}[1][\taskind]{\sma{L\optarg[#1]}}
\newcommand{\envind}{\sma{h}}
\newcommandx{\es}[2][1=\supenvind, 2=\stageind]{\sma{\sigma_{#1}(#2)}}
\newcommandx{\esup}[2][1=\supenvind, 2=\stageind]{\sma{x^{+}_{#1}(#2)}}
\newcommandx{\eslo}[2][1=\supenvind, 2=\stageind]{\sma{x^{-}_{#1}(#2)}}

\newcommandx{\esuplo}[2][1=\supenvind, 2=\stageind]{\sma{x^{\pm}_{#1}(#2)}}

\newcommandx{\eres}[1][1=\supenvind]{\sma{R_{#1}}}
\newcommandx{\eslen}{\sma{\delta}}

%% Stage notation
\newcommand{\stageind}{\sma{h}}
\newcommand{\stages}[1][\taskind]{\sma{M\optarg[#1]}}

\newcommandx{\stage}[3][1=\taskind, 2=\envind, 3={,}]{\sma{\sigma_{#1#3#2}}}
\newcommandx{\sres}[2][1=\taskind, 2=\envind]{\sma{R_{#1,#2}}}
\newcommandx{\slen}[2][1=\taskind, 2=\envind]{\sma{t_{#1,#2}}}

%% Per-stage number of memory transactions: generic, read, write
\newcommandx{\mtr}[2][1=\taskind, 2=\envind]{\sma{\mu^r_{#1,#2}}}
\newcommandx{\mtw}[2][1=\taskind, 2=\envind]{\sma{\mu^w_{#1,#2}}}
\newcommandx{\mt}[2][1=\taskind, 2=\envind]{\sma{\mu_{#1,#2}}}

%% Per-stage bandwidth: generic, read , write
\newcommandx{\bwr}[3][1=\taskind, 2=\envind, 3={,}]{\sma{b^r_{#1#3#2}}}
\newcommandx{\bww}[3][1=\taskind, 2=\envind, 3={,}]{\sma{b^w_{#1#3#2}}}
\newcommandx{\bw}[3][1=\taskind, 2=\envind, 3={,}]{\sma{b_{#1#3#2}}}

%% Task parameters
\newcommand{\per}[1][\taskind]{\sma{T\optarg[#1]}}
\newcommand{\dead}[1][\taskind]{\sma{D\optarg[#1]}}
\newcommand{\wcet}[1][\taskind]{\sma{C\optarg[#1]}}

%% Global system parameters
\newcommand{\mgp}{\sma{P}}
\newcommand{\mgb}[1][\cpuind]{\sma{Q\optarg[#1]}}
\newcommand{\mgbovh}[1][\cpuind]{\sma{Q'\optarg[#1]}}

%% MemGuard Overhead Cycles
\newcommand{\ovht}{\sma{t_{ovh}}}
\newcommand{\ovhx}{\sma{x_{ovh}}}

%% Profile notation
\newcommand{\sampind}{\envind}
\newcommand{\runind}{\sma{r}}

\newcommandx{\samp}[2][1=\sampind, 2=\runind]{\sma{s_#2(#1)}}
\newcommandx{\sampt}[2][1=\sampind, 2=\runind]{\sma{s^t_#2\optpar[#1]}}
\newcommandx{\sampw}[2][1=\sampind, 2=\runind]{\sma{s^w_#2\optpar[#1]}}
\newcommandx{\sampr}[2][1=\sampind, 2=\runind]{\sma{s^r_#2\optpar[#1]}}
\newcommandx{\sampu}[2][1=\sampind, 2=\runind]{\sma{s^u_#2\optpar[#1]}}

\newcommand{\sampravg}[1][\sampind]{\sma{\bar{b}^r\optpar[#1]}}
\newcommand{\sampwavg}[1][\sampind]{\sma{\bar{b}^w\optpar[#1]}}
\newcommand{\sampavg}[1][\sampind]{\sma{\bar{b}\optpar[#1]}}

\newcommand{\cutoff}{\sma{\beta}}

%% Slopes and intercepts for MG utilization model
\newcommand{\mguslope}{\sma{U^{k}_{mg}}}
\newcommand{\mguicep}{\sma{U^{a}_{mg}}}

%% Slopes and intercepts for QoS utilization model
\newcommandx{\quslope}[1][1=w]{\sma{U^{k}_{qos,#1}}}
\newcommandx{\quicep}[1][1=w]{\sma{U^{a}_{qos,#1}}}

%% QoS settings paramters
\newcommandx{\fclk}{\sma{f_{clk}}}
\newcommandx{\qoslev}[1][1=\accind]{\sma{Q\optarg[#1]}}
\newcommandx{\qosarr}{\texttt{ar\_r}\xspace}
\newcommandx{\qosawr}{\texttt{aw\_r}\xspace}

\newcommandx{\qosarb}{\texttt{ar\_b}\xspace}
\newcommandx{\qosawb}{\texttt{aw\_b}\xspace}

\newcommandx{\qosarp}{\texttt{ar\_p}\xspace}
\newcommandx{\qosawp}{\texttt{aw\_p}\xspace}

\newcommandx{\qoswsize}{\texttt{w}\xspace}
\newcommandx{\qosbww}[1][1=w]{\sma{b_{qos,#1}}}

==> docs/old-1-introduction.tex <==
osection{Introduction}\label{intro}


\begin{figure*}[]
  \centering
  \includegraphics[width=0.95\textwidth]{figs/vision-blackbox.pdf}
  \caption{Motivation, black-box model \textcolor{red}{Will be replaced with a better quality}}
  \label{fig:flow}
\end{figure*}


\todo{(idealistic graph) Plot to compare y-axis: latency   x-axis: level of projectivity   later follows}

Over the past few years, the popularity of large scale real-time analytics of data has gone sky high with the advent of big data. Hence many of the modern-day applications require the ability to perform both online transaction processing (
  OLTP) and online analytical processing (OLAP) within the same database. However, 
  OLTP and OLAP systems have very different properties. 
  OLTP systems are generally optimized for write-intensive workloads by optimizing high volume of point access queries using indexes. In contrast, OLAP systems are optimized for read-only queries that access large amounts of data. Most OLAP systems store data in a columnar fashion that supports fast-scan of data. Because of the contrast in their properties, designing a database engine supporting both workloads is challenging. 
The term Hybrid Transactional/Analytical Processing (HTAP) represents the class of systems that support both transactional and analytical processing on the same database. In order to bridge the requirements of 
OLTP and OLAP, many HTAP systems use a single architecture that ingests data in 
row-format and once data hit the disc convert them into a columnar format. By doing this, HTAP systems fuse the pipelines of ingesting data and performing analytics which leads to a single data-store maintaining the fresh data along with efficient analytics on that same data set. Because of the massive increase of HTAP workloads in recent years, HTAP systems have gained considerable attractions from both industry and academia.

A lot of hybrid approaches have been proposed that try and bridge the benefits of both OLTP and OLAP systems. These systems can be broadly classified into two groups: (1) systems that use the same data representation for both OLTP and OLAP and (2) systems that use different data representation. Almost all of the systems belonging to the former group (H2TAP~\cite{appuswamy2017case}, Hyper~\cite{kemper2011hyper}, L-Store~\cite{sadoghi2016store}, etc.) are optimized for one type of processing and later added support for the other type of processing. On the other hand, the latter group (SAP HANA~\cite{farber2012sap}, MemSQL~\cite{memsql}, IBM dashDB~\cite{dashdb}, Pelaton~\cite{pavlo2017self} etc.) employs various different techniques to store data in hybrid layouts. \textcolor{blue}{Modern hardware impact?} But defining and maintaining these layouts carries a large amount of extra complexity, which leads to runtime inefficiency and heavy book-keeping overheads. However, with the growth of main memory capacity, the transformation cost is becoming the bottleneck for fast analytics. \textcolor{blue}{out-of-sync.} In addition, the database community has seen an explosion of in-memory database systems like VoltDB~\cite{stonebraker2013voltdb}, Hekaton~\cite{diaconu2013hekaton} etc. All of the aforementioned sub-optimal designs can be pinpointed to one issue, i.e. that data is essentially stored in one physical layout. While some designs store data in multiple layouts, they do so through replication which comes with several complications like properly maintaining data copies, buffer management and space amplification.

One of the key bottlenecks in modern computing is moving the data through the memory hierarchy to the processor(s), which serve(s) as the ``central'' units that execute logic and perform computation.
% Traditional computing architectures have been built around a processor-centric paradigm. CPUs are ``central'' units towards which data needs to be transported for computation to occur. 
Motivated by the performance gap between processors and DRAM memory technology, multi-level caches have been introduced to hide the latency of memory fetches. The resulting memory hierarchy can exhibit good performance under the assumption that access to data is characterized by \textit{spatial} and \textit{temporal} locality. 

This assumption, however, is not valid even in an approximate sense for data-intensive workloads, like tensor and image processing, machine learning, database systems, and large-scale data analytics, to name a few. In data-intensive workloads, processing is performed by streaming over a set of data items that is (1) orders of magnitude larger than the typical size of CPU caches; (2) often sparsely stored in memory; and (3) accessed with hard to predict, input-dependent patterns that are not optimized for the 
row/column organization of data in DRAM. To make things worse, as data is streamed through the processors, the amount of computation performed on each data item may be minimal. Thus, hiding the latency of data movement via deep pipelines and instruction-level reordering becomes harder, if not impossible. Data movement is the key bottleneck in data-driven workloads.  Importantly, data movement in modern processors represents an important portion of the overall power draw.  Hence, compressing the amount of data moved between processors and DRAM will have an important impact on overall energy consumption.

To address this problem, traditional architectural paradigms need to be revisited. The traditional angle under which the problem of data-intensive processing has been approached is via accelerators. Accelerators represent additional processing elements specialized for the type of data computation required for a domain-specific type of workload. The boost in performance achieved via accelerators, however, is offset by the additional complexity in (1) seamlessly integrating support for multiple ISAs within the same compilation toolchain, and in (2) supporting the interaction between main processors and multiple accelerators at the level of the OS.

In this paper, we explore a different angle in approaching the problem of optimizing data-intensive workloads. We propose to alternate between (1) performing computation closer to data for processing steps with poor data locality; and (2) re-organize and compress data items as they are moved towards the CPUs to improve locality; and (3) use traditional CPUs for processing steps after good data locality has been enforced. This can be done by {\bf departing from the traditional view of main memory as a flat array of bytes}. Instead, we propose introducing some amount of near-memory computation to re-organize, pre-filter and pre-process data before it is moved to the central processing units. \textcolor{blue}{Little bit more details about PLIM.} In other words, we propose exploiting the inherent parallelism of memory cells (e.g. multiple DRAM banks, DRAM rows with larger width than what is strictly required for bus transactions and cache line-fills) to perform computation that would exhibit poor locality when moved to the CPUs as is. Once data has been reorganized to improve its locality, main CPUs can be used as needed. Further, we envision that online data re-organization and final processing can be \textbf{concurrently performed in a pipelined fashion}, thus boosting the achievable speedup even further.

In this paper, we will consider commercially available SoCs that include programmable logic (PL) and a traditional multi-core (MC) processor on the same chip.  We will refer to these SoCs as MC+PL SoCs. In MC+PL SoCs it is already possible to instantiate logic that acts as an intermediary between embedded processors and main memory. By sitting between CPUs and main memory, we achieve a new degree of control over memory transactions, with an approach we call \emph{Programmable Logic In-the-Middle} (PLIM) ~\cite{roozkhosh2020potential}. The PLIM approach opens up new avenues to design and deploy resource management primitives previously available only through hardware re-design. It also creates new opportunities in the definition of OS-level and hypervisor-level technologies that leverage PLIM modules to improve performance management, self-awareness, and online workload characterization. In addition, by employing commercial MC+PL SoCs it is possible to create usable proof-of-concept prototypes to assess performance benefits with realistic applications.




\todo{(idealistic graph) Plot to compare y-axis: latency   x-axis: level of projectivity   later follows by the realistic plot}


